The End of a Black Hole's Evaporation -- Part I

At the end of Hawking evaporation, the horizon of a black hole enters a physical region where quantum gravity cannot be neglected. The physics of this region has not been much explored. We characterise its physics and introduce a technique to study it.

==> B transition Part 1 2/config.tex <==

\pdfoutput=1

% for quotation marks (english style)
\usepackage[autostyle, english = british]{csquotes}
\MakeOuterQuote{"}

\usepackage[english]{babel}

\usepackage{graphicx}
\usepackage{adjustbox}
\usepackage{subfigure}
\usepackage{capt-of}
\usepackage{amsmath,amssymb,amsfonts,tensor}
\usepackage{xcolor}

\usepackage{physics} % for \bracket \matrixel \Re \Im
\usepackage[percent]{overpic} %writing over pictures

\usepackage[colorlinks,citecolor=blue,linkcolor=blue,urlcolor=blue,pdfencoding=auto, psdextra]{hyperref}
%\usepackage[applemac]{inputenc}


\setlength{\paperheight}{11in}  %to avoid hyperref warning

%definitions
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand*{\diff}{\mathop{}\!\mathrm{d}}

